Upside-Down Reinforcement Learning for More Interpretable Optimal Control

Model-Free Reinforcement Learning (RL) algorithms either learn how to map states to expected rewards or search for policies that can maximize a certain performance function. Model-Based algorithms instead, aim to learn an approximation of the underlying model of the RL environment and then use it in combination with planning algorithms. Upside-Down Reinforcement Learning (UDRL) is a novel learning paradigm that aims to learn how to predict actions from states and desired commands. This task is formulated as a Supervised Learning problem and has successfully been tackled by Neural Networks (NNs). In this paper, we investigate whether function approximation algorithms other than NNs can also be used within a UDRL framework. Our experiments, performed over several popular optimal control benchmarks, show that tree-based methods like Random Forests and Extremely Randomized Trees can perform just as well as NNs with the significant benefit of resulting in policies that are inherently more interpretable than NNs, therefore paving the way for more transparent, safe, and robust RL.

==> Plots/importance_feature.tex <==

\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Plots/feature_viz/CartPole-v0/RandomForestClassifier/env_image_1.png} 
    \end{subfigure}    
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                ylabel={Importance},
                grid=both,
                width=\textwidth,
                height=0.9\textwidth,
                xtick=data,
                xticklabels={\(x\), \(\dot{x}\),\(\theta\),\(\dot{\theta}\), $d_r$, $d_h$},
                x tick label style={rotate=45, anchor=east},
                enlarge x limits=0.05,
                ybar,
                bar width=10pt,
                error bars/y dir=both,
                error bars/y explicit
            ]
            \addplot[fill=red, draw=red] table {Plots/feature_viz/CartPole-v0/RandomForestClassifier/info_1.dat};
            
        \end{axis}
        \end{tikzpicture}
        \caption{Cartpole}
    \end{subfigure}
    \caption{Overall figure caption}
\end{figure}


\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Plots/feature_viz/Acrobot-v1/RandomForestClassifier/env_image_0.png} 
    \end{subfigure}    
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                ylabel={Importance},
                grid=both,
                width=\textwidth,
                height=0.9\textwidth,
                xtick=data,
                xticklabels={\(\sin{\theta_1}\),\(\cos{\theta_1}\),\(\sin{\theta_2}\),\(\cos{\theta_2}\),\(\dot{\theta}_1\),\(\dot{\theta}_2\),$d_r$, $d_h$},
                x tick label style={rotate=45, anchor=east},
                enlarge x limits=0.05,
                ybar,
                bar width=10pt,
                error bars/y dir=both,
                error bars/y explicit
            ]
            \addplot[fill=red, draw=red] table {Plots/feature_viz/Acrobot-v1/RandomForestClassifier/info_0.dat};
            
        \end{axis}
        \end{tikzpicture}
        \caption{Cartpole}
    \end{subfigure}
    \caption{Overall figure caption}
\end{figure}


\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Plots/feature_viz/LunarLander-v2/RandomForestClassifier/env_image_0.png} 
    \end{subfigure}    
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                ylabel={Importance},
                grid=both,
                width=\textwidth,
                height=0.9\textwidth,
                xtick=data,
                xticklabels={
                \(x\),\(y\),\(\dot{x}\),\(\dot{y}\),\(\theta\),\(\dot{\theta}\),$lc$,$rc$,$d_r$, $d_h$},
                x tick label style={rotate=45, anchor=east},
                enlarge x limits=0.05,
                ybar,
                bar width=10pt,
                error bars/y dir=both,
                error bars/y explicit
            ]
            \addplot[fill=red, draw=red] table {Plots/feature_viz/LunarLander-v2/RandomForestClassifier/info_1.dat};
            
        \end{axis}
        \end{tikzpicture}
        \caption{Cartpole}
    \end{subfigure}
    \caption{Overall figure caption}
\end{figure}



==> Plots/results.tex <==
\begin{figure*}[htbp]
    \centering
    % First subfigure (CartPole)
    \begin{subfigure}{0.32\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                title={\texttt{CartPole}},
                width=\linewidth,
                height=\linewidth,
                xlabel={Episode},
                ylabel={Reward},
                ymin=0, ymax=200,
                xtick={0, 500, 1000, 1500, 2000},
                ytick={0, 100, 200},
                grid=both,
                major grid style={line width=0.8pt, draw=gray!70},
                minor grid style={line width=0.4pt, draw=gray!50},
                minor x tick num=4, % Creates minor ticks every 50 episodes
                minor y tick num=2, % Creates minor ticks every 50 units on the y-axis
                style={line width=2pt}, % Thicker lines
                ]
                \addplot+[smooth, color=blue!50, mark=none] table [col sep=comma, x=episode, y=NN_mean_smoothed] {Results/CartPole-v0.csv};
                \addplot+[smooth, color=green!50, mark=none] table [col sep=comma, x=episode, y=RF_mean_smoothed] {Results/CartPole-v0.csv};
                \addplot+[smooth, color=red!50, mark=none] table [col sep=comma, x=episode, y=ET_mean_smoothed] {Results/CartPole-v0.csv};
                \addplot+[smooth, color=purple!50, mark=none] table [col sep=comma, x=episode, y=KNN_mean_smoothed] {Results/CartPole-v0.csv};
                \addplot+[smooth, color=orange!50, mark=none] table [col sep=comma, x=episode, y=AdaBoost_mean_smoothed] {Results/CartPole-v0.csv};
                \addplot+[smooth, color=cyan!50, mark=none] table [col sep=comma, x=episode, y=XGBoost_mean_smoothed] {Results/CartPole-v0.csv};
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}%
    % Second subfigure (Acrobot)
    \begin{subfigure}{0.32\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                title={Acrobot},
                width=\linewidth,
                height=\linewidth,
                xlabel={Episode},
                ylabel={Reward},
                ymin=-500, ymax=-50,
                xtick={0, 500, 1000, 1500, 2000},
                ytick={-500, -200, -50},
                grid=both,
                major grid style={line width=0.8pt, draw=gray!70},
                minor grid style={line width=0.4pt, draw=gray!50},
                minor x tick num=4, % Creates minor ticks every 50 episodes
                minor y tick num=4, % Creates minor ticks every 50 units on the y-axis
                style={line width=2pt}, % Thicker lines
                ]
                \addplot+[smooth, color=blue!50, mark=none] table [col sep=comma, x=episode, y=NN_mean_smoothed] {Results/Acrobot-v1.csv};
                \addplot+[smooth, color=green!50, mark=none] table [col sep=comma, x=episode, y=RF_mean_smoothed] {Results/Acrobot-v1.csv};
                \addplot+[smooth, color=red!50, mark=none] table [col sep=comma, x=episode, y=ET_mean_smoothed] {Results/Acrobot-v1.csv};
                \addplot+[smooth, color=purple!50, mark=none] table [col sep=comma, x=episode, y=KNN_mean_smoothed] {Results/Acrobot-v1.csv};
                \addplot+[smooth, color=orange!50, mark=none] table [col sep=comma, x=episode, y=AdaBoost_mean_smoothed] {Results/Acrobot-v1.csv};
                \addplot+[smooth, color=cyan!50, mark=none] table [col sep=comma, x=episode, y=XGBoost_mean_smoothed] {Results/Acrobot-v1.csv};
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}%
    % Third subfigure (LunarLander)
    \begin{subfigure}{0.32\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                title={LunarLander},
                width=\linewidth,
                height=\linewidth,
                xlabel={Episode},
                ylabel={Reward},
                ymin=-350, ymax=0,
                xtick={0, 500, 1000, 1500, 2000},
                ytick={-500, -200, 0},
                grid=both,
                major grid style={line width=0.8pt, draw=gray!70},
                minor grid style={line width=0.4pt, draw=gray!50},
                minor x tick num=4, % Creates minor ticks every 50 episodes
                minor y tick num=4, % Creates minor ticks every 50 units on the y-axis
                style={line width=2pt}, % Thicker lines
                ]
                \addplot+[smooth, color=blue!50, mark=none] table [col sep=comma, x=episode, y=NN_mean_smoothed] {Results/LunarLander-v2.csv};
                \addplot+[smooth, color=green!50, mark=none] table [col sep=comma, x=episode, y=RF_mean_smoothed] {Results/LunarLander-v2.csv};
                \addplot+[smooth, color=red!50, mark=none] table [col sep=comma, x=episode, y=ET_mean_smoothed] {Results/LunarLander-v2.csv};
                \addplot+[smooth, color=purple!50, mark=none] table [col sep=comma, x=episode, y=KNN_mean_smoothed] {Results/LunarLander-v2.csv};
                \addplot+[smooth, color=orange!50, mark=none] table [col sep=comma, x=episode, y=AdaBoost_mean_smoothed] {Results/LunarLander-v2.csv};
                \addplot+[smooth, color=cyan!50, mark=none] table [col sep=comma, x=episode, y=XGBoost_mean_smoothed] {Results/LunarLander-v2.csv};
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}
    
    \vspace{0.5cm} % Add some space before the legend
    
    % Add legend below all subfigures
    \begin{minipage}{\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                axis y line=none,
                axis x line=none,
                width=0.9\textwidth,
                height=0.2\textwidth,
                legend columns=3, % 3 columns for the legend
                legend style={at={(0.5,1)}, anchor=north, column sep=1ex, font=\footnotesize, legend cell align=left},
                ]
                \addplot+[color=blue!50, mark=none] coordinates {(0,0)}; \addlegendentry{NN}
                \addplot+[color=green!50, mark=none] coordinates {(0,0)}; \addlegendentry{RF}
                \addplot+[color=red!50, mark=none] coordinates {(0,0)}; \addlegendentry{ET}
                \addplot+[color=purple!50, mark=none] coordinates {(0,0)}; \addlegendentry{KNN}
                \addplot+[color=orange!50, mark=none] coordinates {(0,0)}; \addlegendentry{AdaBoost}
                \addplot+[color=cyan!50, mark=none] coordinates {(0,0)}; \addlegendentry{XGBoost}
            \end{axis}
        \end{tikzpicture}
    \end{minipage}

    \caption{Comparison of the performance of various models (NN, RF, ET, KNN, AdaBoost, and XGBoost) on three OpenAI Gym environments: CartPole, Acrobot, and LunarLander. The results are shown in terms of smoothed rewards per episode. \textbf{Best viewed in color.}}
    \label{fig:comparison}
\end{figure*}


==> Tables/environments.tex <==
\begin{table*}[h!]
\centering
\scriptsize
\caption{MDP Description of the CartPole, Acrobot, and Lunar Lander Environments}
\begin{tabular}{>{\columncolor[HTML]{EFEFEF}}l p{4cm} p{4cm} p{4cm}} % Adjusted the width for each column
\toprule
\textbf{Component} & \texttt{CartPole} & \texttt{Acrobot} & \texttt{Lunar Lander} \\ \midrule
\textbf{States} \(\mathcal{S}\) & 
\begin{tabular}[t]{@{}l@{}} 
Continuous 4D vector: \\ 
- \(x\): Cart Position  \\ 
- \(\dot{x}\): Cart Velocity  \\ 
- \(\theta\): Pole Angle \\ 
- \(\dot{\theta}\): Pole Angular Velocity
\end{tabular} & 
\begin{tabular}[t]{@{}l@{}} 
Continuous 6D vector: \\ 
- \(\sin{\theta_1}\): Sine of the first link \\ 
- \(\cos{\theta_1}\): Cosine of the first link \\ 
- \(\sin{\theta_2}\): Sine of the second link \\ 
- \(\cos{\theta_2}\): Cosine of the second link \\ 
- \(\dot{\theta}_1\): Angular velocity of first link \\ 
- \(\dot{\theta}_2\): Angular velocity of second link
\end{tabular} & 
\begin{tabular}[t]{@{}l@{}} 
Continuous 8D vector: \\ 
- \(x\): X position \\ 
- \(y\): Y position \\ 
- \(\dot{x}\): X linear velocity \\ 
- \(\dot{y}\): Y linear velocity \\ 
- \(\theta\): Angle \\ 
- \(\dot{\theta}\): Angular velocity \\ 
- Left and right leg contact points
\end{tabular} \\ \midrule

\textbf{Actions} \(\mathcal{A}\) & 
\begin{tabular}[t]{@{}l@{}} 
Discrete: \\ 
0: Push left \\ 
1: Push right 
\end{tabular} & 
\begin{tabular}[t]{@{}l@{}} 
Discrete: \\ 
0: Torque left \\ 
1: No torque \\ 
2: Torque right 
\end{tabular} & 
\begin{tabular}[t]{@{}l@{}} 
Discrete: \\ 
0: Do nothing \\ 
1: Fire left engine \\ 
2: Fire main engine \\ 
3: Fire right engine 
\end{tabular} \\ \midrule

\textbf{Rewards} $r_t$ & 
+1 for every step taken & 
-1 for every step until the goal is reached & 
\begin{tabular}[t]{@{}l@{}} 
+100 for successful landing \\ 
-100 for crash landing \\ 
Reward for firing engines and leg contact
\end{tabular} \\ \bottomrule
\end{tabular}
\label{tab:MDPEnvironments}
\end{table*}

==> Tables/inference_commands.tex <==
\begin{table}[htbp] 
\caption{}
\centering
\scriptsize
\begin{tabular}{>{\columncolor[HTML]{EFEFEF}}lcccc}
\toprule
\textbf{Behaviour Function} & \texttt{CartPole}   & \texttt{Acrobot}   & \texttt{Lunar Lander}   \\ \midrule
Neural Network     & & &  &      \\ 
Random Forest      & & &  &      \\  
Extra-Trees     & & &  &      \\     
KNN    & & &  &      \\ 
AdaBoost     & & &  &      \\ 
XGBoost     & & &  &      \\ 
\bottomrule
\end{tabular}
\label{tab:inference_parameters}
\end{table}

==> Tables/results.tex <==
%% REMEMBER:
%%% Results calculated on the best seed with the best desired horizon and desired returns. 
%%% Median +- STD is shown 
%%% Best seed is decided using a score function which is:
%%% score = median*0.5 + mean*0.1 + 1/(1+std*0.3) + 1/(1+range*0.1)
%%% Only the seed with the highest score is shown in the table 


\begin{table*}[htbp]
\caption{The results of the six tested behavior functions obtained at inference time, namely when the behavior function $f$ gets queried with the desired reward $d_t$ and desired horizon $d_h$ commands described in Table \ref{}. The best performing algorithm is reported in a green cell, whereas the second best performing algorithm is reported in a yellow cell.}
\centering
% Second identical table
\begin{tabular}{>{\columncolor[HTML]{EFEFEF}}lcccc}
\toprule
\textbf{Behaviour Function} & \texttt{CartPole}   & \texttt{Acrobot}   & \texttt{Lunar Lander}   \\ \midrule
Neural Network     & $199.93 \pm 0.255$ &$-75.00 \pm 15.36$ & $-157.04 \pm 71.26$ &      \\ 
Random Forest      &$188.25 \pm 13.82$ &$-100.05 \pm 15.36$ &$-54.74 \pm 96.22$ &      \\ 
Extra-Trees     &$181.56 \pm 31.63$ & $ -100.00 \pm 93.72$& $-127.79 \pm49.19$&      \\
KNN    & $85.11\pm50.30$ &$-160.50 \pm 36.66$  & $-128.47\pm47.49 $&      \\
AdaBoost     & $168.61\pm31.02$ & $-109.00\pm63.70$& $-108.26\pm80.71$ &      \\
XGBoost     &$199.27\pm4.06$&$-100.00\pm34.71$ &$-76.96\pm89.69$ &      \\
\bottomrule
\end{tabular}
\end{table*}


